AMS-KV: Adaptive KV Caching in Multi-Scale Visual Autoregressive Transformers

Visual autoregressive modeling (VAR) via next-scale prediction has emerged as a scalable image generation paradigm. While Key and Value (KV) caching in large language models (LLMs) has been extensively studied, next-scale prediction presents unique challenges, and KV caching design for next-scale based VAR transformers remains largely unexplored. A major bottleneck is the excessive KV memory growth with the increasing number of scales-severely limiting scalability. Our systematic investigation reveals that: (1) Attending to tokens from local scales significantly contributes to generation quality (2) Allocating a small amount of memory for the coarsest scales, termed as condensed scales, stabilizes multi-scale image generation (3) Strong KV similarity across finer scales is predominantly observed in cache-efficient layers, whereas cache-demanding layers exhibit weaker inter-scale similarity. Based on the observations, we introduce AMS-KV, a scale-adaptive KV caching policy for next-scale prediction in VAR models. AMS-KV prioritizes storing KVs from condensed and local scales, preserving the most relevant tokens to maintain generation quality. It further optimizes KV cache utilization and computational efficiency identifying cache-demanding layers through inter-scale similarity analysis. Compared to the vanilla next-scale prediction-based VAR models, AMS-KV reduces KV cache usage by up to 84.83% and self-attention latency by 60.48%. Moreover, when the baseline VAR-d30 model encounters out-of-memory failures at a batch size of 128, AMS-KV enables stable scaling to a batch size of 256 with improved throughput.

==> Tables/model_spec.tex <==
\begin{table}[t]
    \centering
    \caption{Model specifications with different configurations.}
    \label{tab:model_specs}
    \begin{tabular}{l|ccccc}
        \toprule
        \textbf{Model} & \textbf{Layers} & \textbf{Params.} & \textbf{Heads} & \textbf{Dims} & \textbf{$C_{cds}$} \\
        \midrule
        VAR-d12  & 12  & -      &  -     & xx & 5\\
        VAR-d16  & 16  & 310M   &  16   & 1024 & 5\\
        VAR-d20  & 20  & 600M   &  20   & 1280 & 5\\
        VAR-d24  & 24  & 1.0B   &  24   & 1536 & 5\\
        VAR-d30  & 30  & 2.0B   &  30   & 1920 & 5\\
        VAR-d36  & 36  & -      &  -    & yy & 5\\
        \bottomrule
    \end{tabular}
\end{table}
